El Agente: An Autonomous Agent for Quantum Chemistry

Computational chemistry tools are widely used to study the behaviour of chemical phenomena. Yet, the complexity of these tools can make them inaccessible to non-specialists and challenging even for experts. In this work, we introduce El Agente Q, an LLM-based multi-agent system that dynamically generates and executes quantum chemistry workflows from natural language user prompts. The system is built on a novel cognitive architecture featuring a hierarchical memory framework that enables flexible task decomposition, adaptive tool selection, post-analysis, and autonomous file handling and submission. El Agente Q is benchmarked on six university-level course exercises and two case studies, demonstrating robust problem-solving performance (averaging >87% task success) and adaptive error handling through in situ debugging. It also supports longer-term, multi-step task execution for more complex workflows, while maintaining transparency through detailed action trace logs. Together, these capabilities lay the foundation for increasingly autonomous and accessible quantum chemistry.

==> editing_commands.tex <==

\usepackage{soul, color}
\newcommand{\Note}[1]{}
\renewcommand{\Note}[1]{#1}  %
\newcommand{\NoteSigned}[3]{{\textcolor{#2}{\Note{\textbf{[#1: #3]}}}}}

\newcommand{\pl}[1]{\NoteSigned{PL}{blue}{#1}}  %
\newcommand{\tc}[1]{\NoteSigned{TC}{green}{#1}}
\newcommand{\cb}[1]{\NoteSigned{CB}{brown}{#1}}
\newcommand{\cj}[1]{\NoteSigned{CJ}{purple}{#1}}
\newcommand{\sm}[1]{\NoteSigned{SM}{magenta}{#1}}
\newcommand{\aa}[1]{\NoteSigned{AA:}{orange}{#1}}
\newcommand{\jz}[1]{\NoteSigned{JZ:}{cyan}{#1}}


\newcommand{\itodo}[1]{\NoteSigned{TODO}{red}{#1}}
\newcommand{\prelim}[1]{\NoteSigned{Prelim}{grey}{#1}}

\newcommand{\sowhat}{$\rightarrow$~}

\newcommand{\aagcomment}[1]{\NoteSigned{AAG}{green}{#1}} 

\newcommand{\bluebox}[1]{\todo[color=blue!20!white]{#1}}

